Learning Incident Prediction Models Over Large Geographical Areas for Emergency Response Systems

Principled decision making in emergency response management necessitates the use of statistical models that predict the spatial-temporal likelihood of incident occurrence. These statistical models are then used for proactive stationing which allocates first responders across the spatial area in order to reduce overall response time. Traditional methods that simply aggregate past incidents over space and time fail to make useful short-term predictions when the spatial region is large and focused on fine-grained spatial entities like interstate highway networks. This is partially due to the sparsity of incidents with respect to the area in consideration. Further, accidents are affected by several covariates, and collecting, cleaning, and managing multiple streams of data from various sources is challenging for large spatial areas. In this paper, we highlight how this problem is being solved for the state of Tennessee, a state in the USA with a total area of over 100,000 sq. km. Our pipeline, based on a combination of synthetic resampling, non-spatial clustering, and learning from data can efficiently forecast the spatial and temporal dynamics of accident occurrence, even under sparse conditions. In the paper, we describe our pipeline that uses data related to roadway geometry, weather, historical accidents, and real-time traffic congestion to aid accident forecasting. To understand how our forecasting model can affect allocation and dispatch, we improve upon a classical resource allocation approach. Experimental results show that our approach can significantly reduce response times in the field in comparison with current approaches followed by first responders.

==> sayyed_paper_text.tex <==
\section{Problem Statement/Formulation}  \label{Problem Statement}
The problem to be addressed is designing a model imitating the real incident occurrence, which can be used in ERM pipeline to optimize the allocation and dispatching the responders. The most conventional method is hotspot analysis, which evaluates the spatial distribution of the accidents ~\cite{cheng2005experimental,yu2014comparative,ryder2019spatial}. While it is relatively simple and fast, it does not consider the temporal effects. Linear regression models are the other convectional methods for incident occurrence prediction. While the most common one is linear regression model with Gaussian errors~\cite{frantzeskakis1994interurban,jovanis1986modeling}, they usually incapable of incorporating the sporadic nature of emergency incidents~\cite{miaou1993modeling,joshua1990estimating}. Thanks to the aggregation techniques, linear regression models can be more accurate \cite{rakha2010linear}. The accident occurrence cannot be negative and linear regression models are not able to address that. To solve this problem,  Poisson models were suggested \cite{jovanis1986modeling,sayed1999accident,joshua1990estimating}. A Poisson assumes the expected value of the response variable and the variance of that are equal, which may be violated in accident dataset. Therefore, Poisson-hierarchical models, such as  Poisson-gamma,  Poisson-lognormal, and Poisson-inverse-gamma, were used \cite{Deublein2013, Quddus2008, akinCrashBinomial, ladron2004forecasting, ackaah2011crash, Shirazi2019,  Aguero-ValverdeJonathan2013FBPg, Khazraee2018}. As it is explained later, a big challenge is usually the sparsity of the data. To overcome this problem, zero-inflated models were introduced \cite{qin2004selecting,lord2007further,huang2010modeling,lord2005poisson}. In the recent years, due to the huge amount of data collected from various sensors, data mining models have gained more attention. Neural networks~\cite{Pande2006,Abdelwahab2002,Chang2005,Riviere2006,zhu2018use,Bao2019}, support vector machine~\cite{doi:10.3141/2024-11,Li2008,Yu2013}, and random forests~\cite{Abdel-Aty2008,Yu2014} are some of the most important ones. Most of the aforementioned studies are either just spatial or the time resolution is coarse, which makes it fruitless for ERM purposes. Furthermore, the papers aiming to improve ERM are heavily focused on allocation and dispatching model rather than accident prediction part (for further information please refer to \cite{mukhopadhyay2020review},) while even the proposed dispatching and allocated model are too complicated or problem-specific to be employed by organization. For example, the allocation and dispatching model is used by TDOT is far from the state of the art. Therefore, one of the goals of this paper is to present an simple and accurate enough pipeline as well prediction model, than can simply be employed. Furthermore,  this method alongside the non-complicated convectional allocation and dispatching models should show a tangible improvement.




Learning models over emergency incident occurrence is a challenging task for two main reasons --- first, such incidents have been known to be inherently random, and second, despite their alarming numbers, incidents are very sporadic when viewed from the perspective of total time and space. Depends on the goal and application as well as the time and space resolution, the employed method may vary. We may discretize the space, time, or both. The range for the size of time discretization may vary from hour to a year or even more. Assume if the goal is to study the influence of rush hour on the total number of accidents which may require hourly time frames while if the goal is to evaluate the effect of a pandemic on the macro accident rate pattern which the window may be as wide as a month or a year. Space discretizition is not different. We may want to analyze the accident patterns in an intersection or in a city.  Obviously, temporal and spatial discretizition may be applied to the problem simultaneously. 


Considering the extent of the time and space, an accident is inherently a very rare event. Therefore, the probability of accident occurrence in a short time frame and on a small segment of a highway is virtually zero. In other words, if we discretize time and space, depending on the size of  discretizition, most of the spatial temporal grids do not incorporate any accidents. By increasing the size of the grids, moving from finer mesh to a coarser mesh, the number of the spatial temporal grids with no accident shrinks.
%\ref{fig:schematic_sparisty} schematically shows the number of accidents per roadway segment (space) and time window, which is called \emph{cell} hereafter. roadway segment can be defined using Open Street Map (OSM)  \cite{4653466} and window can be defined by splitting a day into six 4-hour window.


%As mentioned earlier, the prime application of resource demand models, incident prediction, is to strategically distribute the resources, responders. Therefore, the developed model should be spatial temporal with a high resolution using macro level data, which is not an easy task. 




\subsection{Formulation}  \label{Formulation}
Considering $\mathcal{S}$ as the space domain and $\mathcal{T}$ as the time domain,  in general, the goal is to develop a model $f$ based on historical accidents $\mathbf{x_i},  \forall i \in 1,2,\dots, N$, where $N$ is the total number of accidents in $\mathcal{S}$ and $\mathcal{T}$; environmental features $\mathbf{W_j} \in \mathbbm{R}^{S \cdot T}$, $\forall j \in 1,2,\dots, M$, where $M$ is the total number of features as well as $S$ and $T$ are the size of $\mathcal{S}$ and $\mathcal{T}$, respectively; and learning parameters $\theta$ to predict a measure of incident occurrence $y_{s,t}$, such as rate or chance of accidents, in location $s \in \mathcal{S}$ and time $t \in  \mathcal{T}$:

%\begin{equation} \label{eq1}
%\mathbf{y}=f(\mathbf{s},\mathbf{t} \mid \mathbf{x}, \mathbf{W},\theta)
%\end{equation}


\begin{equation} \label{eq2}
y_{s,t}=f(s,t \mid \mathbf{x}, \mathbf{W},\theta)
\end{equation}


In this paper, we aim to  design a pipeline and train a model that can predict the probability of occurrence of incident in the unit of time and space. Time unit is 4-hour windows. Space unit is based on the INRIX roadway segmentation. If at least one accident happens during the 4-hour time window $t$ on the roadway segment $s$, which is called \emph{cell} of $t$ and $s$ hereafter, occurrence value, $y$, for that \emph{cell} would be \emph{one} otherwise it would be \emph{zero}. The prediction model estimates the probability of the occurrence of incident for a \emph{cell}: $P({y=1 \mid s,t})$

In our problem, $\mathcal{S}$ is highway segment of the State of Tennessee, and  $(\mathcal{T}$) is from 2017 to 2020, which are discussed later in the case study. Considering the 4-hour time window, 2190 windows exist in a year, and for about 4 years of data $S \approx 8,500$. The historical accident records for about 5,000 roadway segment is available; $T \approx 8,500$. Total number of the accidents for this $\mathcal{S}$ and $\mathcal{T}$ is about 80,000.







%The features regarding the accident $\mathbf{x}_i$ can be represented by the tuple $\{\mathbf{s}_i,\mathbf{t}_i,\mathbf{w}_i\}$, where $\mathbf{s}_i$ and $\mathbf{t}_i$ denote the location (spatial feature) and time (temporal feature) of the occurrence, respectively. $\mathbf{w}_i \in \mathbb{R}^m$ represents a vector of features associated with the incident. The typical features that can be included in $\mathbf{w}$  are weather information, traffic flow, the number of the lanes, etc. The goal is to develop a model $f$ based on historical accidents $\mathbf{x}$ and  learning the parameters $\theta$, which can be formulated by $f(\mathbf{y} \mid \mathbf{x},\theta)$, to predict a measure of incident occurrence $\mathbf{y_j}$, such as rate of accidents location $\mathbf{s}_j$ and time $\mathbf{t}_j$. 



\textcolor{green}{SMV: We can add some other studies here}


\subsection{Sparsity Problem}  \label{Problem Statement}
Learning models over emergency incident occurrence is a challenging task for two main reasons --- first, such incidents have been known to be inherently random, and second, despite their alarming numbers, incidents are very sporadic when viewed from the perspective of total time and space. Depends on the goal and application as well as the time and space resolution, the employed method may vary. We may discretize the space, time, or both. The range for the size of time discretization may vary from hour to a year or even more. Assume if the goal is to study the influence of rush hour on the total number of accidents which may require hourly time frames while if the goal is to evaluate the effect of a pandemic on the macro accident rate pattern which the window may be as wide as a month or a year. Space discretizition is not different. We may want to analyze the accident patterns in an intersection or in a city.  Obviously, temporal and spatial discretizition may apply to the problem simultaneously. Considering the extent of the time and space, an accident is inherently a very rare event. Therefore, the probability of accident occurrence in a short time frame and on a small segment of a highway is virtually zero. In other words, if we discretize time and space, depending on the size of  discretizition, most of the spatial temporal grids do not incorporate any accidents. By increasing the size of the grids, moving from finer mesh to a coarser mesh, the number of the spatial temporal grids with no accident shrinks.
Figure \ref{fig:schematic_sparisty} schematically the sparsity of the problem. 
Since showing all segments and all time windows in one figure is not possible, Figure \ref{fig:schematic_sparisty} illustrates 180 randomly selected roadway segments for April 2019. Totally 32400 $cells$ exist in this figure. If accident occurred in a $cell$, it is shown in white, otherwise it remains black. As it can be seen most of the figure is black and just 67 $cells$ are white; about 0.2\% of the total number of cells. Although Figure \ref{fig:schematic_sparisty} is drawn just for one month of data and limited number of roadway segments, it gives us an overview of the sparsity level. The total sparsity level is 0.2065\%.

shows the number of accidents per roadway segment (space) and time window, which is called \emph{cell} hereafter. roadway segment can be defined using Open Street Map (OSM)  \cite{4653466} and window can be defined by splitting a day into six 4-hour window.

\begin{figure}[h!]
\centering
\includegraphics[width=2.5in]{images/schematic_sparisty_2.png}
\caption{Schematic overview of the sparsity of accident occurrence}
\label{fig:schematic_sparisty}
\end{figure}





\subsubsection{Accuracy of the Model}

\textcolor{red} {SMV: I think using figures such as the following one would be so helpful to explain the metrics. However, bringing up this figure falls into the section results. Furthemore, maybe we dont have to explain all the metrics since most of them are familiar to readers. We should just focus on the Distance metric.}

\paragraph{Lay-out of the figures}: Figure \ref{fig:lay_out} shows a lay out for the visualization of the prediction results. In the Central part which is bounded by a blue box, the spatio temporal distribution of probability of accident occurrence is shown, similar to Figure \ref{fig:schematic_sparisty}.  Right part and the top part, the yellow boxes, are the marginal distribution of accident occurrence given time, $P({y=1 \mid t})$, and the marginal distribution of accident occurrence given space, $P({y=1 \mid s})$, respectively. The top right of the figure, the green square, shows the total average. Finally, on the left side of side, the red box, the clusters are color coded, if the prediction model uses a clustering technique. This lay out would be preserved for illustrating the accuracy of the models and comparing them. 


For example, Figure \ref{fig:Spatial_Tempral} a and b are generated by the real data and the prediction probability, respectively. Since all the segments are time windows cannot fit in one figure, some of them are randomly selected. The results are based on the test dataset, which means the trained models has never seen them before. %In the central part of each one, the x-axis and y-axis indicate time (4-hour window) and space (roadway segment), respectively. 
In figure \ref{fig:Spatial_Tempral} a, if accident occurs in a \emph{cell}, that \emph{cell} is shown in white otherwise it is black. However, in figure \ref{fig:Spatial_Tempral} b, the \emph{cell} are color coded based on the predicted probability of occurrence of accident. The blue \emph{cells}, are the missing \emph{cells}, due to a missing value in the features. By comparing the cluster box and the marginal distribution of accident occurrence given space, in \ref{fig:Spatial_Tempral} b, it can be seen, the segments belong to cluster one (yellow) have higher average likelihood compare those of belong to the purple cluster (cluster zero).



\paragraph{Spearman Correlation of the Spatial Marginal Distributions}:

\begin{figure}[h!]
\centering
\includegraphics[width=1.5in]{images/lay_out.png}
\caption{Lay out}
\label{fig:lay_out}
\end{figure}


\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/Spatial_Tempral.png}
\caption{Spatial Temporal Distribution of the accident occurrence}
\label{fig:Spatial_Tempral}
\end{figure}



If we can predict the hourly accident rate for the whole highways in the state of Tennessee, it would be ideal. However, on average, in year 2018, less than 3 accidents happened per hour in the highways of Tennessee \textcolor{green}{SMV:I can elaborate more on it using figures and numbers; however, if I say something more then it need to define the segments, grouping, cells, etc.}. It clearly shows the sparsity level of the accident data. Furthermore, they are various factors, including the environment, the roadway, the driver and the vehicle, etc that contribute to road accidents. Combination of all these factors and complexity of collecting data on all the factors make analyzing of roadway car accidents to be a nontrivial problem. Because of the complexity of the problem in a very fine temporal spatial discretizition, accident events act similar to a random event; predicting the hourly accident rate for a segment which has had just one accident during last couple of years is not feasible or we can just consider it as zero. Considering the sparisty and inherent random nature of the problem, it is virtually impossible to predict the accident rate at this resolution for all over the Tennessee.


Furthermore, based on the application prediction various metrics can be employed to evaluate the performance of the model. 


\paragraph{Accuracy, precision, recall, and F1-score}
Accuracy, precision, recall, and F1-score are common factors can be drived from the cinfusion matrix. For unbalanced classification problems the importance of F1-score is even more. Otherwise, due to the sparsity of the problem, any prediction model that always predicts zero can be 99.2\% of the time correct which results in a very high accuracy number. Even though all of the aforementioned values are reported, the focus will be on F1-score. 


\paragraph{Correlation}
Calculating the correlation of marginal distribution of accident occurrence given space for predicted data and the real data can be a factory of accuracy. In general, we expet the model to predict higher chance of accidents for the segments they have a higher average rate of accident occurrence. This goal can be achieved by Pearson correlation. However, for the sake of completeness and not being limited to just linear correlation, Spearman correlation is also reported.  


\paragraph{Likelihood}

\paragraph{Travel Distance}
The most accurate way to evaluate the performance of the prediction in practice is to evaluate the model for an actual scenario. In other words, the model should be evaluated compared to the current approach used by TDOT. The current method is used by TDOT is to draw a spatial heatmap and allocate the responders according to that. The location of the responders do not change over time. However, using our prediction model, the location of the responders can be redesigned every four hours. In order to reduce the influence of allocation model, the same allocation model is used for both models. Furthermore, the allocation model should be relatively similar to what is used by TDOT. Moreover, the allocation model should be simple and fast to be useful for a real time ERM. A modified version of P-median problem is considered for allocation model and the method suggested by ??? is used to solve the problem \cite{???}.  

an allocation be represented as $\min_{y} G(y \mid f)$, where $y$ is the decision variable (location of responders), $G$ is a cost function, and $f$ is the model of incident occurrence. For allocation problems. Here the cost function is $ Cost= \sum_{i=1}^{i=n} \sum_{j=1}^{j=m} d_{ij} k_{ij} p_{i} b_{j}$, where $n$  and $m$ are the number of segments and responders, respectively. $ d_{ij}$ is the distance between segment $i$  and responder $j$. $k_{ij}$ is a binary value that indicates if responder $j$ is the closest responder to segment $i$. $p_{i}$ is the chance of accident occurrence on segment $i$. $b$ is a balance factor to penalize the responders are supposed to be dispatched to more potential accidents; $b_{j}= {(\frac{\sum_{i=1}^{i=n} k_{ij} p_{i}}{\sum_{i=1}^{i=n} p_{i}})^\alpha}$, and $\alpha$ is a weight parameter; by increasing $\alpha$ this ratio becomes more influential. In summary, solving this optimization problems, positions the responders closer to the segments with higher chance of accidents while putting more responders in the dense regions. Figure \ref{fig:allocation.png} schematically shows the optimum allocation scenarios using $\alpha=0$  on the left and $\alpha=2$ on the right, the numbers in the cells shows with chance of accident.


\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/allocation.png}
\caption{Schematic responders allocations for different alternatives}
\label{fig:allocation.png}
\end{figure}



Based on prediction model, a predefined numbers of responders are distributed on the map by the allocation model. Then we run real scenario for each four-hour time slots in the test data. Whenever an accident occurs, the closest available responders is dispatched to that accident, and that responder will be unavailable for an hour after that. one hour is the average time that it takes for a responder to arrive at the location of accident, take care of the situation, and come back to the station to be available for the next mission. At the end of each four-hour time slots, we calculate the total travel distance. In some rare cases scenarios, there may not be any available responders to be dispatched. In that case, we consider a penalty value. The same total travel distance is calculated using the allocation based on a spatial heatmap, which TDOT is currently using.  Subsequently, we can compare the average of the total travel distances to see if the prediction model can reduce the travel distance by the responders. 






\section{Data Preparation} \label{Data Preparation}

The accuracy of models highly depends on the input data features. The features can be collected or stratigically generated. Also, the availability of features may limit the type of models that can be used. In general, features can be categorized into temporal, spatial, or combination of both. Features can be created from the available features by applying mathematical functions on them or combining them. 


\subsection{Data Sources} \label{Data Sources}
In this research, various sources are used to collect the required data. In the following section, each source is discussed. Apart from the sources mentioned below, other sources are also investigated but the following ones are chosen due the accuracy, compatibility, or other factors. For example, for the weather data, both weatherbit and darksky were investigated; however, since the dataset based on darksky suffered from more missing values for the intended time time and spacial region, weatherbit was selected. Another example is the option to choose the roadway segment features available through ETRIMS. Even though ETRIMS provides some features that INRIX does not such as AADT, but cannot be useful due to the lack of accuracy and incompatibility with the traffic data. Figure \ref{fig:ETRIMS_vs_INRIX.png} shows the available roadway segments available through INRIX and ETRIMS in red and green, respectively. The location of the accidents are also marked in blue. As it an be seen ETRIMS provides one line representing both bounds, which will result in erroneous prediction results. 


\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/ETRIMS_vs_INRIX.png}
\caption{Comparing the quality of the roadway segments available through INRIX and ETRIMS}
\label{fig:ETRIMS_vs_INRIX.png}
\end{figure}


\begin{itemize}
 \item Roadway information: The majority of the data regarding roadways are collected from INRIX. It provides location-based data and analytics, such as roadway segments and traffic. Based on INRIX, about 80,000 main roadway segments exist in Tennessee, and about 20,000 of them are highway segments. The static features a roadway segment incorporate the coordinates, length, number of the lanes, etc. These features do not change over time or the change is negligible. Traffic is a spacio-termporal feature, which also also extracted over time through INRIX. The traffic information for segments in 5-minute time resolution is available since April/2017. The traffic information for a segment includes the free flow speed, the estimated current speed, time it will take to drive along the roadway segment, confidence score, and so forth. Due to the the number of the segments and the aforementioned time resolution, the size of this dataset is more than 1.2TB. \textcolor{green}{SMV: I dont know if it is necessary to mention what challenges this data may create} \textcolor{green}{SMV: should we mention the problems we encountered by using etrims?}
 
 \item Weather information: Weather is inherently spatial temporal, and can play an important role in accident rates. The information includes temperature, precipitation, visibility, etc. The hourly weather information is collected from the weatherbit.io. To predict the weather all over Tennessee 40 different stations are available. The geographical locations of the stations is shown in figure \ref{fig:weather_stations}. \textcolor{green}{SMV: should we mention the problems we encountered by using darksky?} 
 

\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/weatherbit.png}
\caption{Location of the weather stations}
\label{fig:weather_stations}
\end{figure}
 
 \item Incident Features: Through our collaboration with the Tennessee Department of Transportation (TDOT), we gained access to the state of Tennessee's incident records spanning from January 2017 to May 2020. This consists of approximately 78,000 accidents once filtered to only incidents which occurred on highways. These records included the location and time each incident occurred, as well as features such as the number and severity of reported injuries and the number of involved vehicles. 
 
\end{itemize} 



\subsection{Grouping} \label{Grouping} 



\subsection{Features} \label{Feature} 


\begin{itemize}
 \item Temporal Features: Also, temporal features can play a key role so features such as time of the day and being weekend or not are also considered. It has been proven that historical data is a crucial factor in prediction of the total number of accidents \cite{mukhopadhyay2020review}. 
 In order to incorporate that into the problem, the number of accidents in the past time windows for the intended segment is extracted. In other words, features such as the total number of accidents in the exact previous time window, a day before, a week before, etc. are used. 
 
 \item Spatio-Temporal Features: Weather and traffic data are generally considered as spatio-temporal features. Some of the features such as temperature, precipitation, and visibility are available directly while some other features such as congestion are available indirectly from one the resources mentioned above. The latter category requires some extra steps which is explained in the next section. features extracted based  
 
 \item Spatial Features: Spatial features are mostly limited to the features regarding the geometry or location of the roadways. In this study features such as number of the lanes and length of the segment are available directly and used in the model. Some other features such as iSF (inverse Shape Factor) are extracted based on the geometry features of the road, which is explained in the next section. 
 
 

 
 %In other words, if a segment has a high rate of accident there is high chance the neighbouring segments also have a high rate of accidents. The table below, summarizes all the features. The other important factor worth mentioning is the effect of adjacent segments on each other.


 
\end{itemize} 

\subsubsection{Feature Creation} \label{Feature Creation} 
The following features are extracted indirectly from one of the above mentioned sources.

\begin{itemize}
 \item iSF: We introduce a feature to represent horizontal turns in the models, which is called on inverse stretch factor (iSF). Stretch Factor is defined as the ratio of the length of the curve to the shortest path between the two ends of the curve. ISF is the inverse of Stretch Factor and takes a value between 0 and 1. 1 is a straight line, 0 is almost a closed shape. Figure \ref{fig:ISF} shows a segment in TN, where iSF is the length the straight line AB over the of curve AB.  Another alternatives are  curvature \cite{Wang2009}, bend \cite{Deublein2013}, bend density and detour ratio \cite{Haynes2007}.


 \begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/isf.png}
\caption{length of a curve and the shortest path between the two ends of the curve}
\label{fig:ISF}
\end{figure}
 
 %We consider the minimum and end to end value for each segment. For vertical changes, we consider median of the slope and end to end slope for each segment. 
 
  %is the curvature of the roadway. However, the complete geometry of the roadway is not available. In fact, just the coordinates of the a few points from the roadway is available, which makes extracting the curvature unreliable. 
 
 
 \item Congestion: This feature is calculated by the difference between the free flow speed and the current speed over the free flow speed of the roadway. If the current speed is bigger than the free flow speed we just simply assign zero for the congestion value. 
 

 \end{itemize} 

 
 
 \subsection{Data cleaning} \label{Data cleaning} 
 Similar to any real data, the data requires a lot efforts to be cleaned. The datasets are collected from various resources which they should be combined. Therefore, they should convert to a compatible format. Furthermore, the quality of the datasets are comporised my missing and erroneous values. For example, the incident dataset from TDOT has also some features regarding the weather. However, there are obvious conflicts between the weather information on the accident report  and weatherbit. Comparing with a third source of weather data, we concluded that the weatherbit dataset is more reliable. 


\input{tables/table1}
 
 \subsection{Combining the Datasets} \label{Combining the Datasets}  
 First, the location of the incidents are mapped to the roadway segments. By having the coordinates of the incidents as a point and roadway segments as one or multiple lines, the incidents are assigned to the closest segment unless the distance is more than 25 meters. By doing so, less than 1\% of the accident data remains unassigned mostly due to erroneous coordinates or being incorrectly categorized as highway incidents while they are not. The roadways segments presented by INRIX will be are spatial dimension. The weather data for each roadway segments is collected from the one of the 40 available stations based on the closest distance. Since both traffic dataset and roadway dataset extracted from INRIX, using just the ID of the segment traffic can be easily mapped to the roadway segments. This part can be called spatial mapping. The other dimension is time. Each day is dived into six equal  4-hour windows; Midnight to 4:00 a.m., 4:00 a.m. to 8:00 am, and so on. By doing so, a year , with 365 days, is break into 2190 4-hour time windows. Since the weather dataset is hourly and traffic data set is 5-minute resolution, these two datasets are aggregated for 4-h to match the base spatial resolution. At the end of this step, a dataset is available which incorporates all of the aforementioned datasets in a spatial-termporal manner. 
 
 
 
 \textcolor{red} {The features are used for prediction in this study are as follows, weekend or not (0 or 1), number of the window of the day (0,1,2,3,4,5), precipitation, visibility, temperature, iSF, congestion, number of the lanes, length of the segments, number of the accident in the day before at the exact same window, number of the accident on the day before, number of the accident on 7 days earlier at the exact same window, number of the accident in last 7 days, ...}
 
 
 
 
 
 
 
 
 
 

\section{Resource Demand Models} \label{Resource Demand Models}
The main problem we are aiming to solve is to estimate the number of accidents (or accident rate) in both time (window) and space (segment). As discussed earlier, accident events in this resolution are very rare events; therefore, there are just very few cells whose number of accidents are not zero, and even fewer cells have more than one accident. Considering that, the problem can be simplified to just two classes: cells with no accidents and cells with at least one accident. Consequently, the problem is modified to a binary classification problem.



\subsection{Our Solution}
The problem can be considered as a two-unbalanced-class classification problem. If the features introduced in the previous sections are not sufficient for a binary classification problem, most likely they are not sufficient for a prediction rate problem either. If there is one accident on a highway segment during the last 3 years, it is virtually impossible to predict an accident occurrence prediction for that segment using such short historical data. Therefore, in order the lower the sparsity level of the problem, we choose the top $20\%$ groups of the segments with the highest non-zero \emph{cells}, accounting for 78\% of all accidents. Using various techniques, the accuracy of each method is investigated.  


\subsubsection{Addressing the Sparsity}
As mentioned earlier, the problem is very sparse; there are a lot of segments with no accident in a 4-hour window. In order to improve the quality of the model, the data should be less sparse. The following procedures are employed to reduce the sparsity level of the problem without comprising the accuracy. 
\paragraph{Grouping}
The roadway segment defined by INRIX compose the spatial unit of the problem. Some of the segments might be very short resulting in a very low chance of accident, In order to reduce the sparsity of the problem, we combine similar neighboring segments using a procedure called grouping. After this step, and selecting the top 20\% groups with highest accident occurrence, the non-sparsity level increases from 0.25\% to 2.27\%.

\paragraph{Resampling}
This problem in nature is an unbalanced spatial-temporal classification problem. \emph{Class I} includes the \emph{cells}  with no accident while \emph{Class II} are the \emph{cells}  with at least one accident. However, most of the \emph{cells}  fall into the former category. Therefore, the it is an unbalanced classification problem. To help the model to predict more accurately,  different strategies can be adopted, includeding various resampling methods. Random Over Sampling (ROS) and Random Under Sampling (RUS) are among the most common methods.  \textcolor{red} {We should add some references}
\paragraph{Clustering}
Not all the roadway segments follow the same behaviour. Therefore, it is required to train different models for different behaviours. The similar segments, which is expected to have similar accident pattern, are clustered together. Here, the similarity feature is considered to be the average accident rate in the training dataset. Having, $n$ clusters, $n$ separate models are trained. Among all various types of clustering, K-means is used due to the simplicity. 

\subsubsection{Regression Models}
Among the regression models, logistic regression is used for predicting the accident occurrence. The advantage of this method is its simplicity and speed. However, it might be flexible enough to provide accurate result. First a simple logistic regression model is applied on the clustered data. Using train data the model is trained and using the verification data the threshold is adjusted. Subsequently, in two separate analyses, a simple logistic regression is applied on the clustered and then resampled (ROS and RUS).
\paragraph{Logistic Regression}
\paragraph{Logistic Regression for unbalanced data}

\subsubsection{NN}
\subsubsection{Tree based}
\subsubsection{SVM}




\subsection{Pipeline/Tool chain}  \label{Pipeline}
The pipeline is summarized in Figure  \ref{fig:pipeline}. First the datasets are collected from various resources and are cleaned. Afterwards, during the spatial mapping, the accidents are assigned to their closest roadways segments, and the closest weather station to each roadway segment is determined. Then the main dataframe which is used as the input for the resource demand models is generated. The rows are time and space, \emph{cells}, while the columns are the aggregated features for that \emph{cell}. The output of the prediction models is is a likelihood heatmap, which shows the chance of accident occurrence for each roadway segment.  Then, this heatmap is used by the allocation and dispatch models to distribute the responders on the map. By having the model trained and constantly collecting the data from the environment, the ERM is ready to be used. 

\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/pipeline.png}
\caption{pipelines}
\label{fig:pipeline}
\end{figure}



\section{Discussion and Results}  \label{Discussion and Results}
To generate the following results, the aforementioned method, datasets, and pipeline are employed. 1 month of data is considered as the test data, and from all the available data before that month, 80\% of it is used for training and 20\% is used for verification.  
one month test, 

Figure \ref{fig:map} compares the heatmap of the spatial marginal distribution of accident occurrence for jan/2020 using real data and predicted values. The model is able to imitate the spatial patterns very well, which is important for dispatch modeling. 



\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/map.png}
\caption{map}
\label{fig:map}
\end{figure}




\subsection{Future Work}  \label{Future Work}
Even though the aforementioned process is being evaluated by TDOT to be deployed, there are still some room for improvement. Also, these improvements might be problem specific and may not be applicable to other similar problems. In this problem specifically, due to very limited number of missing data, no measure is taken to fill the missing values,; therefore, the prediction engine does not predict any values for those \emph{cells}. Also, the traffic data is available for some of the roadway segments in five-minute time resolution. Finding  a relationship between anomalies in the traffic flow and accident occurrence can improve the accuracy of the results. However, due to the complexity and broadness of this problem, it can be a separate research topic on its own. Furthermore, it is worth mentioning, the accuracy of this data-driven model can improve by continuous data collection. This allows us to incorporate unusual conditions such as COVID-19 pandemic, which changed the traffic and accident patterns. 

\#\#\#\#weather


\section{Implementation}  \label{Implimentation} 



\subsubsection{Dashboard}  \label{Dashboard}
Figure \ref{fig:dashboard} shows a screen shot of the dashboard created by the authors for this project. It shows the heatmap of the accidents on the map for a range of time. Also, it shows the distribution of of accidents over time, for example comparing the number of accidents per month, per day of the week, or time of the day. Furthermore, the aforementioned figures can be regenerated based on filter features . For instance, the the distribution of the accidents in a rainy day is of interest, the data can be filtered by the feature precipitation. This dashboard is very helpful to understand the importance of the features and distribution of the accidents over time and space, which will be used by the allocation and dispatch models. 
\begin{figure}[h!]
\centering
\includegraphics[width=3in]{images/dashboard.png}
\caption{dashboard}
\label{fig:dashboard}
\end{figure}






\section{Conclusion}
has yet to be completed.

==> tables/missed_accident_BW.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\captionsetup{font=small}
\centering
\caption{Average and maximum number accidents in each 4-h window that responders are not able to immediately respond because all responders are busy (the best performance in each column is shown in bold text)}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{8}{c|}{average number of   unattended accidents} & \multicolumn{8}{c|}{maximum number of   unattended accidents} \\ \hline
\multicolumn{1}{|c|}{\textbf{$p$}} & \multicolumn{4}{c|}{\textbf{10}} & \multicolumn{4}{c|}{\textbf{15}} & \multicolumn{4}{c|}{\textbf{10}} & \multicolumn{4}{c|}{\textbf{15}} \\ \hline
\multicolumn{1}{|c|}{\textbf{$\alpha$}} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} \\ \hline
Naive & 0.54 & 0.49 & 0.48 & 0.46 & 0.02 & 0.01 & 0.01 & 0.01 & 15.00 & 14.00 & 14.00 & 16.00 & 2.00 & 1.00 & 1.00 & 2.00 \\ \hline
LR+NoR+NoC1 & 0.54 & 0.47 & 0.42 & 0.42 & \textbf{0.00} & \textbf{0.00} & 0.01 & 0.01 & 16.00 & 13.00 & 14.00 & 12.00 & \textbf{0.00} & \textbf{0.00} & 1.00 & 1.00 \\ \hline
LR+RUS+NoC1 & 0.56 & 0.52 & 0.46 & 0.46 & \textbf{0.00} & \textbf{0.00} & 0.01 & \textbf{0.00} & 17.00 & 17.00 & 15.00 & 15.00 & \textbf{0.00} & \textbf{0.00} & 1.00 & \textbf{0.00} \\ \hline
LR+ROS+NoC1 & 0.56 & 0.51 & 0.46 & 0.45 & \textbf{0.00} & \textbf{0.00} & 0.01 & \textbf{0.00} & 17.00 & 17.00 & 15.00 & 14.00 & \textbf{0.00} & \textbf{0.00} & 1.00 & \textbf{0.00} \\ \hline
LR+NoR+KM2 & 0.53 & 0.41 & 0.43 & 0.44 & 0.02 & 0.01 & 0.01 & 0.01 & 17.00 & 12.00 & 13.00 & 15.00 & 3.00 & 1.00 & 1.00 & 2.00 \\ \hline
LR+RUS+KM2 & 0.54 & 0.48 & 0.42 & 0.40 & 0.01 & \textbf{0.00} & \textbf{0.00} & 0.01 & 15.00 & 15.00 & 11.00 & 12.00 & 1.00 & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
LR+ROS+KM2 & 0.54 & 0.48 & 0.42 & 0.41 & 0.01 & \textbf{0.00} & \textbf{0.00} & 0.01 & 15.00 & 15.00 & 11.00 & 15.00 & 1.00 & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
NN+NoR+NoC1 & 0.45 & 0.40 & 0.43 & 0.40 & 0.01 & \textbf{0.00} & 0.01 & 0.01 & \textbf{12.00} & 11.00 & 11.00 & \textbf{11.00} & 1.00 & \textbf{0.00} & 1.00 & 1.00 \\ \hline
NN+RUS+NoC1 & 0.47 & 0.41 & 0.43 & 0.45 & \textbf{0.00} & 0.01 & 0.01 & 0.01 & \textbf{12.00} & 11.00 & 11.00 & 12.00 & \textbf{0.00} & 1.00 & 1.00 & 1.00 \\ \hline
NN+ROS+NoC1 & 0.46 & 0.41 & 0.42 & 0.43 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.01 & \textbf{12.00} & 11.00 & 11.00 & 13.00 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
NN+NoR+KM2 & \textbf{0.44} & 0.40 & 0.42 & 0.42 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 15.00 & 12.00 & 12.00 & 14.00 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} \\ \hline
NN+RUS+KM2 & 0.48 & 0.45 & 0.42 & 0.42 & 0.01 & 0.01 & 0.01 & 0.02 & \textbf{12.00} & 11.00 & 11.00 & 12.00 & 1.00 & 1.00 & 1.00 & 2.00 \\ \hline
NN+ROS+KM2 & 0.48 & 0.41 & 0.44 & 0.41 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.01 & 13.00 & 11.00 & 14.00 & \textbf{11.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
RF+CW+NoC1 & 0.51 & 0.44 & 0.42 & 0.42 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.02 & 13.00 & 12.00 & 12.00 & \textbf{11.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
RF+NoR+NoC1 & 0.48 & 0.40 & \textbf{0.38} & 0.43 & 0.01 & 0.01 & \textbf{0.00} & 0.02 & 13.00 & 12.00 & 13.00 & 13.00 & 1.00 & 1.00 & \textbf{0.00} & 2.00 \\ \hline
RF+RUS+NoC1 & 0.53 & 0.46 & 0.44 & 0.42 & 0.01 & 0.01 & \textbf{0.00} & \textbf{0.00} & 16.00 & 13.00 & 11.00 & 14.00 & 1.00 & 1.00 & \textbf{0.00} & \textbf{0.00} \\ \hline
RF+ROS+NoC1 & 0.46 & 0.41 & 0.40 & 0.41 & 0.01 & 0.01 & \textbf{0.00} & 0.01 & \textbf{12.00} & 11.00 & 12.00 & 12.00 & 1.00 & 1.00 & \textbf{0.00} & 1.00 \\ \hline
RF+CW+KM2 & 0.49 & 0.42 & 0.42 & 0.43 & 0.01 & \textbf{0.00} & \textbf{0.00} & 0.01 & \textbf{12.00} & 13.00 & 11.00 & 12.00 & 1.00 & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
RF+NoR+KM2 & 0.49 & 0.40 & \textbf{0.38} & 0.42 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 13.00 & \textbf{10.00}  & 12.00 & 12.00 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} \\ \hline
RF+RUS+KM2 & 0.51 & 0.45 & 0.43 & 0.40 & 0.01 & \textbf{0.00} & 0.01 & 0.01 & 13.00 & 13.00 & 11.00 & 12.00 & 2.00 & \textbf{0.00} & 1.00 & 1.00 \\ \hline
RF+ROS+KM2 & 0.48 & \textbf{0.38} & \textbf{0.38} & 0.41 & 0.01 & \textbf{0.00} & \textbf{0.00} & 0.01 & \textbf{12.00} & \textbf{10.00}  & \textbf{10.00} & 12.00 & 1.00 & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
ZIP+NoR+NoC1 & 0.51 & 0.45 & 0.41 & 0.40 & 0.02 & \textbf{0.00} & \textbf{0.00} & 0.01 & 12.00 & 15.00 & 12.00 & 14.00 & 3.00 & \textbf{0.00} & \textbf{0.00} & 1.00 \\ \hline
ZIP+RUS+NoC1 & 0.59 & 0.53 & 0.51 & 0.48 & 0.01 & 0.02 & 0.01 & \textbf{0.00} & 16.00 & 17.00 & 15.00 & 15.00 & 2.00 & 3.00 & 2.00 & \textbf{0.00} \\ \hline
ZIP+ROS+NoC1 & 0.59 & 0.53 & 0.51 & 0.48 & 0.01 & 0.02 & 0.01 & \textbf{0.00} & 16.00 & 17.00 & 15.00 & 15.00 & 2.00 & 3.00 & 2.00 & \textbf{0.00} \\ \hline
ZIP+NoR+KM2 & 0.47 & 0.45 & 0.42 & \textbf{0.37} & 0.02 & \textbf{0.00} & 0.01 & 0.01 & 13.00 & 15.00 & 12.00 & 12.00 & 3.00 & \textbf{0.00} & 1.00 & 1.00 \\ \hline
ZIP+RUS+KM2 & 0.55 & 0.48 & 0.49 & 0.46 & \textbf{0.00} & 0.01 & \textbf{0.00} & 0.01 & 16.00 & 13.00 & 15.00 & 12.00 & \textbf{0.00} & 1.00 & \textbf{0.00} & 1.00 \\ \hline
ZIP+ROS+KM2 & 0.57 & 0.49 & 0.48 & 0.45 & \textbf{0.00} & 0.01 & \textbf{0.00} & 0.01 & 17.00 & 13.00 & 15.00 & 12.00 & \textbf{0.00} & 1.00 & \textbf{0.00} & 1.00 \\ \hline
\end{tabular}
}
\label{table:Distance}
\end{table}

==> tables/table_forecasting_BW.tex <==
 
 
 % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Summary of performance evaluation metrics for each model in percentage (the best performance in each column is shown in bold text)}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|c|c|c|c|c|}
\hline
\textbf{Name} & \textbf{Model}       & \textbf{clustering}     & \textbf{Resampling} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Pearson} & \textbf{Spearman} \\ \hline
Naive         & Naive                & No                      & No                  & \textbf{95.5}              & 3.8                & 4.2             & 4.0               & \textbf{82.1}             & 60.8              \\ \hline
LR+NoR+NoC1   & \multirow{6}{*}{LR}  & \multirow{3}{*}{No}     & No                  & 94.0              & 13.8               & 27.4            & 18.2              & 70.4             & 55.2              \\ \cline{1-1} \cline{4-10} 
LR+RUS+NoC1   &                      &                         & RUS                 & 93.0              & 12.8               & 32.3            & 18.3              & 63.1             & 54.7              \\ \cline{1-1} \cline{4-10} 
LR+ROS+NoC1   &                      &                         & ROS                 & 93.0              & 12.8               & 32.3            & 18.3              & 63.2             & 54.7              \\ \cline{1-1} \cline{3-10} 
LR+NoR+KM2    &                      & \multirow{3}{*}{KMeans} & No                  & 93.0              & 12.5               & 30.9            & 17.7              & 76.6             & 58.4              \\ \cline{1-1} \cline{4-10} 
LR+RUS+KM2    &                      &                         & RUS                 & 92.3              & 12.1               & \textbf{34.4}            & 17.8              & 74.2             & 58.1              \\ \cline{1-1} \cline{4-10} 
LR+RUS+KM2    &                      &                         & ROS                 & 92.4              & 12.2               & 34.2            & 17.9              & 74.2             & 58.1              \\ \hline
NN+NoR+NoC1   & \multirow{6}{*}{NN}  & \multirow{3}{*}{No}     & No                  & 94.9              & 19.2               & 32.8            & 24.0              & 71.7             & 58.5              \\ \cline{1-1} \cline{4-10} 
NN+RUS+NoC1   &                      &                         & RUS                 & 95.0              & 19.2               & 32.6            & 24.1              & 73.2             & 59.3              \\ \cline{1-1} \cline{4-10} 
NN+ROS+NoC1   &                      &                         & ROS                 & 94.9              & 19.1               & 32.8            & 23.9              & 69.3             & 54.7              \\ \cline{1-1} \cline{3-10} 
NN+NoR+KM2    &                      & \multirow{3}{*}{KMeans} & No                  & 95.0              & 19.0               & 31.6            & 23.7              & 75.6             & 58.9              \\ \cline{1-1} \cline{4-10} 
NN+RUS+KM2    &                      &                         & RUS                 & 94.7              & 18.4               & 32.7            & 23.3              & 73.1             & 54.6              \\ \cline{1-1} \cline{4-10} 
NN+RUS+KM2    &                      &                         & ROS                 & 94.7              & 18.3               & 33.1            & 23.3              & 74.5             & 55.4              \\ \hline
RF+NoR+NoC1   & \multirow{8}{*}{RF}  & \multirow{4}{*}{No}     & No                  & 95.0              & 19.0               & 31.8            & 23.6              & 78.7             & 63.4              \\ \cline{1-1} \cline{4-10} 
RF+RUS+NoC1   &                      &                         & RUS                 & 95.2              & 19.3               & 30.5            & 23.5              & 67.4             & 56.9              \\ \cline{1-1} \cline{4-10} 
RF+ROS+NoC1   &                      &                         & ROS                 & 95.3              & 18.6               & 25.6            & 22.1              & 79.2             & \textbf{64.6}              \\ \cline{1-1} \cline{4-10} 
RF+CW+NoC1    &                      &                         & Class weights       & 95.4              & \textbf{20.6}               & 30.4            & \textbf{24.4}              & 77.1             & 62.5              \\ \cline{1-1} \cline{3-10} 
RF+NoR+KM2    &                      & \multirow{4}{*}{KMeans} & No                  & 95.1              & 18.9               & 30.5            & 23.2              & 79.8             & 62.3              \\ \cline{1-1} \cline{4-10} 
RF+RUS+KM2    &                      &                         & RUS                 & 95.0              & 19.4               & 32.5            & 24.2              & 73.8             & 57.6              \\ \cline{1-1} \cline{4-10} 
RF+ROS+KM2    &                      &                         & ROS                 & 95.1              & 18.3               & 28.7            & 22.2              & 80.1             & 63.6              \\ \cline{1-1} \cline{4-10} 
RF+CW+KM2     &                      &                         & Class weights       & 95.2              & 19.6               & 30.7            & 23.8              & 72.0             & 59.7              \\ \hline
ZIP+NoR+NoC1  & \multirow{6}{*}{ZIP} & \multirow{3}{*}{No}     & No                  & 94.4              & 14.6               & 26.8            & 18.9              & 74.0             & 58.0              \\ \cline{1-1} \cline{4-10} 
ZIP+RUS+NoC1  &                      &                         & RUS                 & 94.2              & 13.9               & 26.1            & 18.1              & 61.1             & 50.6              \\ \cline{1-1} \cline{4-10} 
ZIP+ROS+NoC1  &                      &                         & ROS                 & 94.2              & 13.9               & 26.7            & 18.2              & 61.2             & 50.6              \\ \cline{1-1} \cline{3-10} 
ZIP+NoR+KM2   &                      & \multirow{3}{*}{KMeans} & No                  & 93.1              & 13.1               & 31.9            & 18.5              & 77.6             & 61.8              \\ \cline{1-1} \cline{4-10} 
ZIP+RUS+KM2   &                      &                         & RUS                 & 93.0              & 12.7               & 30.8            & 17.8              & 74.2             & 57.1              \\ \cline{1-1} \cline{4-10} 
ZIP+RUS+KM2   &                      &                         & ROS                 & 93.0              & 12.8               & 30.9            & 18.0              & 74.3             & 57.0              \\ \hline
\end{tabular}
}
\label{table:performance_evaluation_metrics}
\end{table}
 
 \iffalse
 
\begin{table}[t]
\centering
\caption{Summary of performance evaluation metrics for each model (for each column, the best entry is shown in bold)}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{@{}lllcccccc@{}}
\toprule
Model                 & clustering                    & Resampling      & Accuracy & Precision & Recall & F1-Score & Pearson Correlation & Spearman Correlation   \\ \midrule
Naive                 &-                              &-                & 95.5     & 3.8        & 4.2    & 4.0      & 82.1                & 60.8                   \\\midrule
\multirow{6}{*}{LR}   & \multirow{3}{*}{No  clusters} & No resampling   & 94.0     & 13.8       & 27.4   & 18.2     & 70.4                & 55.2                   \\
                      &                               & RUS             & 93.0     & 12.8       & 32.3   & 18.3     & 63.1                & 54.7                   \\
                      &                               & ROS             & 93.0     & 12.8       & 32.3   & 18.3     & 63.2                & 54.7                   \\
                      & \multirow{3}{*}{clustering}   & No resampling   & 93.0     & 12.5       & 30.9   & 17.7     & 76.6                & 58.4                   \\
                      &                               & RUS             & 92.3     & 12.1       & 34.4   & 17.8     & 74.2                & 58.1                   \\
                      &                               & ROS             & 92.4     & 12.2       & 34.2   & 17.9     & 74.2                & 58.1                   \\\midrule
\multirow{6}{*}{NN}   & \multirow{3}{*}{No  clusters} & No resampling   & 94.9     & 19.2       & 32.8   & 24.0     & 71.7                & 58.5                   \\
                      &                               & RUS             & 95.0     & 19.2       & 32.6   & 24.1     & 73.2                & 59.3                   \\
                      &                               & ROS             & 94.9     & 19.1       & 32.8   & 23.9     & 69.3                & 54.7                   \\
                      & \multirow{3}{*}{clustering}   & No resampling   & 95.0     & 19.0       & 31.6   & 23.7     & 75.6                & 58.9                   \\
                      &                               & RUS             & 94.7     & 18.4       & 32.7   & 23.3     & 73.1                & 54.6                   \\
                      &                               & ROS             & 94.7     & 18.3       & 33.1   & 23.3     & 74.5                & 55.4                   \\\midrule
\multirow{8}{*}{RF}   & \multirow{4}{*}{No  clusters} & No resampling   & 95.0     & 19.0       & 31.8   & 23.6     & 78.7                & 63.4                   \\
                      &                               & RUS             & 95.2     & 19.3       & 30.5   & 23.5     & 67.4                & 56.9                   \\
                      &                               & ROS             & 95.3     & 18.6       & 25.6   & 22.1     & 79.2                & 64.6                   \\
                      &                               & Class weights   & 95.4     & 20.6       & 30.4   & 24.4     & 77.1                & 62.5                   \\
                      & \multirow{4}{*}{clustering}   & No resampling   & 95.1     & 18.9       & 30.5   & 23.2     & 79.8                & 62.3                   \\
                      &                               & RUS             & 95.0     & 19.4       & 32.5   & 24.2     & 73.8                & 57.6                   \\
                      &                               & ROS             & 95.1     & 18.3       & 28.7   & 22.2     & 80.1                & 63.6                   \\
                      &                               & Class weights   & 95.2     & 19.6       & 30.7   & 23.8     & 72.0                & 59.7                   \\\midrule
\multirow{6}{*}{ZIP}  & \multirow{3}{*}{No  clusters} & No resampling   & 94.4     & 14.6       & 26.8   & 18.9     & 74.0                & 58.0                   \\
                      &                               & RUS             & 94.2     & 13.9       & 26.1   & 18.1     & 61.1                & 50.6                   \\
                      &                               & ROS             & 94.2     & 13.9       & 26.7   & 18.2     & 61.2                & 50.6                    \\
                      & \multirow{3}{*}{clustering}   & No resampling   & 93.1     & 13.1       & 31.9   & 18.5     & 77.6                & 61.8                   \\
                      &                               & RUS             & 93.0     & 12.7       & 30.8   & 17.8     & 74.2                & 57.1                   \\
                      &                               & ROS             & 93.0     & 12.8       & 30.9   & 18.0     & 74.3                & 57.0                   \\ \cmidrule(l){1-9} 
\end{tabular}
}
\label{table:performance_evaluation_metrics}
\end{table}
 
 \fi

==> tables/table_response_BW.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\captionsetup{font=small}
\centering
\caption{Average distance (km) that responders travel to reach to the accident scenes in each four hour in January/2020  \textcolor{red}{the various labels to explain the different models are not really explained. The notation needs to be explained}}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{$p$}} & \multicolumn{4}{c}{\textbf{10}}                     & \multicolumn{4}{c}{\textbf{15}}                     & \multicolumn{4}{c}{\textbf{20}}                     & \multirow{2}{*}{Mean} \\ \cmidrule(r){1-13}
\multicolumn{1}{c}{\textbf{$\alpha$}}                      & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} & \textbf{0} & \textbf{0.5} & \textbf{1} & \textbf{2} &                       \\ \cmidrule(l){1-14} 
LR+NoR+KM2                                              & 523        & 492          & 531        & 543        & 327        & 319          & 328        & 335        & 231        & 226          & 223        & 231        & 359                   \\
LR+NoR+NoC1                                             & 539        & 511          & 504        & 546        & 341        & 328          & 337        & 320        & 235        & 192          & 198        & 216        & 356                   \\
LR+ROS+KM2                                              & 560        & 506          & 537        & 540        & 332        & 321          & 330        & 341        & 239        & 222          & 196        & 213        & 361                   \\
LR+ROS+NoC1                                             & 556        & 542          & 506        & 546        & 339        & 328          & 324        & 323        & 239        & 214          & 190        & 218        & 360                   \\
LR+RUS+KM2                                              & 558        & 505          & 533        & 537        & 332        & 321          & 331        & 332        & 240        & 221          & 199        & 215        & 360                   \\
LR+RUS+NoC1                                             & 558        & 532          & 505        & 542        & 339        & 328          & 326        & 318        & 240        & 210          & 193        & 220        & 359                   \\
NN+NoR+KM2                                              & 518        & 500          & 498        & 523        & 307        & 309          & 304        & 328        & 214        & 198          & 193        & 219        & 343                   \\
NN+NoR+NoC1                                             & 478        & 495          & 488        & 527        & 297        & 288          & 297        & 320        & 180        & 185          & 197        & 220        & 331                   \\
NN+ROS+KM2                                              & 510        & 478          & 497        & 556        & 296        & 291          & 304        & 339        & 196        & 193          & 202        & 229        & 341                   \\
NN+ROS+NoC1                                             & 484        & 476          & 498        & 523        & 269        & 285          & 287        & 314        & 177        & 174          & 194        & 220        & 325                   \\
NN+RUS+KM2                                              & 530        & 504          & 501        & 548        & 317        & 321          & 309        & 332        & 200        & 201          & 207        & 233        & 350                   \\
NN+RUS+NoC1                                             & 481        & 490          & 469        & 532        & 290        & 297          & 300        & 331        & 190        & 185          & 191        & 219        & 331                   \\
RF+CW+KM2                                               & 542        & 498          & 497        & 519        & 313        & 294          & 292        & 319        & 205        & 189          & 186        & 218        & 339                   \\
RF+CW+NoC1                                              & 535        & 485          & 490        & 542        & 309        & 295          & 299        & 316        & 202        & 190          & 185        & 219        & 339                   \\
RF+NoR+KM2                                              & 501        & 489          & 495        & 539        & 294        & 296          & 295        & 326        & 187        & 191          & 202        & 225        & 337                   \\
RF+NoR+NoC1                                             & 507        & 486          & 502        & 514        & 305        & 295          & 289        & 330        & 188        & 194          & 193        & 223        & 335                   \\
RF+ROS+KM2                                              & 499        & 490          & 513        & 544        & 308        & 289          & 291        & 324        & 191        & 197          & 205        & 218        & 339                   \\
RF+ROS+NoC1                                             & 513        & 499          & 489        & 538        & 286        & 284          & 293        & 314        & 189        & 183          & 198        & 220        & 334                   \\
RF+RUS+KM2                                              & 541        & 503          & 502        & 538        & 314        & 304          & 307        & 306        & 203        & 186          & 192        & 214        & 342                   \\
RF+RUS+NoC1                                             & 536        & 512          & 504        & 554        & 322        & 300          & 309        & 318        & 222        & 191          & 191        & 219        & 348                   \\
Naive                                                   & 517        & 496          & 533        & 559        & 355        & 320          & 336        & 320        & 240        & 232          & 243        & 255        & 367                   \\ \bottomrule
\end{tabular}
}
\label{table:Distance}
\end{table}
